Bias in Motion: Theoretical Insights into the Dynamics of Bias in SGD Training

Machine learning systems often acquire biases by leveraging undesired features in the data, impacting accuracy variably across different sub-populations. Current understanding of bias formation mostly focuses on the initial and final stages of learning, leaving a gap in knowledge regarding the transient dynamics. To address this gap, this paper explores the evolution of bias in a teacher-student setup modeling different data sub-populations with a Gaussian-mixture model. We provide an analytical description of the stochastic gradient descent dynamics of a linear classifier in this setting, which we prove to be exact in high dimension. Notably, our analysis reveals how different properties of sub-populations influence bias at different timescales, showing a shifting preference of the classifier during training. Applying our findings to fairness and robustness, we delineate how and when heterogeneous data and spurious features can generate and amplify bias. We empirically validate our results in more complex scenarios by training deeper networks on synthetic and real datasets, including CIFAR10, MNIST, and CelebA.

==> NeurIPS2024_Workshop/content.tex <==
\begin{abstract}
Machine learning systems often acquire biases by leveraging undesired features in the data, impacting accuracy variably across different sub-populations.  
%Current understanding of bias formation mostly focuses on the initial and final stages of learning, leaving a gap in knowledge regarding the transient dynamics.
%To address this gap, 
This paper explores the evolution of bias in a teacher-student setup  modeling different data sub-populations with a Gaussian-mixture model, by providing  %We provide 
an analytical description of the stochastic gradient descent dynamics of a linear classifier in this setting.  % which we prove to be exact in high dimension.
%Notably, 
Our analysis reveals how different properties of sub-populations influence bias at different timescales, showing a shifting preference of the classifier during training.  
%Applying our findings to 
%fairness and robustness. %, we delineate how and when heterogeneous data and spurious features can generate and amplify bias.
We empirically validate our results in more complex scenarios by training deeper networks on %synthetic and real 
real datasets including CIFAR10, MNIST, and CelebA. 
\end{abstract}


\section{Introduction}\label{sec:introduction}
\label{introduction}
%Over the past decade, the problem of assessing the fairness of classifiers has garnered significant attention, 
%revealing that 
Machine learning (ML) systems not only reproduce existing biases in the data but also tend to amplify them \cite{kay2015unequal,suresh2021framework,feng2022has}.
Given the complexity of the ML pipeline, isolating and characterising the key drivers of this amplification is challenging. 
%
Theoretical results in this area (e.g., \cite{{sagawa2020investigation,mannelli2022unfair}}) are mostly based on asymptotic analysis, leaving the transient learning regime poorly understood. 
%Due to limitations on computational resources, 
%a trained ML system may operate far from the asymptotic regime and hence existing results may not always apply. Insights from  class imbalance literature~\cite{ye2021procrustean,francazi2023initial} indicate that classifiers converge faster for classes with more data, but how this applies to fairness, where datasets might be balanced by label but imbalanced by demographics, remains unclear. 

Our analysis addresses this gap by providing a precise characterisation of the transient dynamics of online stochastic gradient descent (SGD) in a high dimensional prototypical  model of linear classification. We use the teacher-mixture (TM) framework~\cite{mannelli2022unfair}, where different data sub-populations are modeled with a mixture of Gaussians,  
each having its own linear rule (teacher) for determining the labels. Adjusting the parameters of the data distribution in our framework connects models of fairness and spurious correlations, 
providing a unifying framework and a general set of results applicable to both domains.
Remarkably, our study reveals a rich behaviour divided into three learning phases, where different features of data bias the classifier and causing significant deviations from asymptotic predictions. We reproduce our theoretical findings through numerical experiments in more complex settings, demonstrating validity beyond the simplicity of our model. 



%Our key contributions are: 

%\begin{itemize}
%    \item {\bf High-dimensional analysis}: We demonstrate that in the high-dimensional limit, relevant properties of the classifier, such as the generalisation error, can be expressed using a few sufficient statistics. We prove that their evolution converges to a set of ordinary differential equations (ODEs) that can be solved explicitly in our setting.
    
%    \item {\bf Bias evolution characterisation}: Using our solution, we characterise the evolution of bias throughout training, showing a three-phase learning process where bias exhibits non-monotonic behaviour. Specifically: 
%%        \item {\bf Initial phase}: The classifier is initially influenced by sub-populations with strong class imbalance.
%        \item {\bf Intermediate phase}: The dynamics shifts towards the saliency, or norm, of the samples in a sub-population.
%        \item {\bf Final phase}: Sub-population imbalance, or relative representation, becomes the dominant factor. 
%%    \item {\bf Empirical validation}: We validate and extend our theoretical results through numerical experiments in both synthetic and real datasets, including CIFAR10, MNIST, and CelebA.  
%\end{itemize}
%Altogether, our study reveals a complex time-dependence of learning with structured data that previous theoretical studies have failed to capture. This characterisation is crucial for developing effective bias mitigation strategies, especially under limited computational resources. \stef{add refs to related works in appendix}



\section{Problem setup} 
\label{sec:model}

%{\bf Data distribution.} 
We consider a standard supervised learning setup where the training data consists of pairs 
of a feature vector $\pmb x \in \mathbb{R}^d$ and a binary label $y = \pm 1$.  
To model subgroups within the data \cite{Sagawa2020Distributionally},
we assume that the feature vectors are 
structured as clusters $c_1, \dots, c_m$, 
respectively centered on some fixed attribute vectors $\pmb v_{1}, \cdots ,\pmb v_{m} \in \mathbb{R}^d$. 
Specifically, $\pmb x$ is sampled from a mixture of $m$ isotropic Gaussians:  
\beq \label{eq:inputdist}
\pmb x \sim \sum_{j=1}^m \rho_j \, 
\mathcal{N}(\pmb v_{j} / \sqrt{d},  \Delta_j \mathbb{I}_{d\times d}),
\eeq 
with mixing probabilities $\rho_1, \cdots, \rho_m$ and scalar variances  
$\Delta_1, \cdots, \Delta_m$. Assuming the entries of $\pmb v_{j}$ are of order $1$ as $d$ gets large, the scaling factor $1/\sqrt{d}$  ensures that the Euclidean norm of the renormalised vector is of order $1$. This prevents the problem from becoming either trivial or overly challenging in the high-dimensional limit \cite{lesieur2016phase,lelarge2019asymptotic}.   We adopt a teacher-mixture (TM) scenario \cite{mannelli2022unfair} where each cluster has its own teacher rule:
\beq \label{eq:teacher}
\pmb x \in c_j \quad \Longrightarrow \quad y = \sign(\overline{\pmb w}_j^{\top} \pmb x / \sqrt{d}).
\eeq 
This rule is characterised by the teacher vectors $\overline{\pmb w}_j \in \R^d$, ensuring  linear separability within each cluster.  Fig.~\ref{fig:TM_illustration}b-d illustrate the data distribution for two clusters with opposite mean vectors $\pm \pmb v$, which will be the primary case study for our analysis. 

{\bf Model.} In this study we analyse a linear model applied to the above data distribution. We aim to learn a vector parameter $\pmb w$, referred to as the `student', such that predictions are given by
\beq
\label{eq:student}
\hat{y}(\pmb x) = \pmb w^\top \pmb x/\sd.
\eeq 
The training process involves applying online SGD on the squared loss $\hat{\epsilon} = (y - \hat y)^2$ with learning rate $\eta/2 >0$ (see  Eq.~\ref{eq:w_update} in Appendix \ref{sec:appendix_proof}). 
%At the $k$-th iteration, a feature vector $\pmb x^k$ is sampled from (\ref{eq:inputdist}), the ground truth label $y^k$ and current model prediction $\hat y^k$ are respectively given by (\ref{eq:teacher}) and (\ref{eq:student}), and the parameter is updated as:
%\beq
%\label{eq:w_update}
%\Delta \pmb w^{k} := 
%\pmb w^{k+1} - \pmb w^k = - \frac{\eta}{2}\nabla {\hat \epsilon}^k(\pmb w^{k}) =  \frac{\eta}{\sqrt{d}} (y^k - \hat y^k) \, \pmb x^k 
%\eeq 
In our analysis, the model is evaluated by its generalisation error, or population loss, $\epsilon := \mathbb{E} [\hat{\epsilon}]$. 

\section{SGD analysis}

\begin{figure*}[t]
    \vskip 0.2in
    \begin{center}
        \begin{subfigure}[b]{0.30\textwidth}
            \centering
            \includegraphics[width=\textwidth]{NeurIPS2024/figures_main/fig1d.pdf}
            \caption{ODEs vs simulations}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.2\textwidth}
            \centering
            \includegraphics[width=\textwidth]{NeurIPS2024/figures_main/fig1c.pdf}
            \vspace{0.3cm}
            \caption{Robustness model}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.2\textwidth}
            \centering
            \includegraphics[width=\textwidth]{NeurIPS2024/figures_main/fig1b.pdf}
            \vspace{0.3cm}
            \caption{Centered fairness}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.2\textwidth}
            \centering
            \includegraphics[width=\textwidth]{NeurIPS2024/figures_main/fig1a.pdf}
            \vspace{0.3cm}
            \caption{General fairness}
        \end{subfigure}
        \caption{
        \textbf{Teacher-Mixture in fairness and robustness.} 
        \textit{Panel (a)} shows the generalisation errors---for the subpopulations $+$ (blue) and $-$ (red)---obtained through simulation (crosses) and predicted by the theory (solid lines) for a network with linear activation. The inset shows the same comparison for the \textit{order parameters}: $R_+$ (blue), $R_-$ (red), $M$ (green), and $Q$ (orange). 
        \textit{Panels (b-d)} exemplify the different scenarios achievable in the TM model investigated in Sec.~\ref{sec:insights}.
        \textit{Panel (b)} represent a model for robustness where a spurious feature---given by the shift vector---can mislead the classifier, see Sec.~\ref{sec:spurious}.
        \textit{Panels (c,d)} are instead discussed in Sec.~\ref{sec:fairness} and represent two models of fairness. First, \textit{Panel (c)} has no shift, $v=0$, allowing us to remove the confounding effects. Finally, \textit{Panel (d)} shows the general fairness problem.
        }
        \label{fig:TM_illustration}
    \end{center}
    \vskip -0.2in
\end{figure*}

\label{sec:SGD}
We study the evolution of the generalisation error 
during training %with SGD with constant learning rate 
in the high dimensional setting (i.e. large $d$). 
Following a classical approach \cite{saad1995dynamics,biehl1995learning}, we streamline the problem by focusing on a small set of summary statistics, referred to as `order parameters', which fully characterises the dynamics.  As the dimension increases, it can be shown by concentration arguments that the evolution of these order parameters converges to the deterministic solution of a system of ODEs \cite{goldt2019dynamics,ben2022high, 
arnaboldi2023high}. 
Notably, in our setting, 
we achieve an analytical solution of this ODE system. 
%We sketch our main results below, referring to the Appendix for derivations and proofs.  

\subsection{Order parameters}  

In the setup described in Section \ref{sec:model}, consider the following 
$2m+1$ variables: 
\beq \label{eq:oparam}
R_j = \frac1d\w^\top \overline{\w}_j, \quad M_j = \frac1d \w^\top  \v_j, \quad Q = \frac1d\|\w\|^2,
\eeq 
for $1\leq j \leq m$. These variables correspond to key statistics of the student, namely its  alignment  to the cluster teachers, its alignment to the cluster centers, and its magnitude,  respectively. Lemma \ref{thm:gen_error} in Appendix \ref{sec:appendix_proof} 
shows how the generalisation error depend on the model parameter $\pmb w$ only through these order parameters. 



\subsection{High dimensional dynamics}
\label{sec:solvingODE}

Let $\mathcal S:=(S_i)_{1\leq i \leq2m+1}$ denote the collection of order parameters. Theorem \ref{thm:concentration_ODEs} in Appendix \ref{sec:appendix_proof} states that as $d$ gets large, the stochastic evolution $\mathcal S^k$ of the order parameter gets uniformly close, with high probability,  to the average continuous-time dynamics described by the ODE system: 
\beq \label{eq:gen_ODE}
\frac{d\bar{\mathcal S}_i(t)}{dt} = f_{i}(\bar{\mathcal S}(t)), \qquad 1\leq i \leq 2m+1,
\eeq 
where  the  continuous \textit{time} is given by the example number divided by the input dimension, $t=k/d$.

{\bf Solving the ODEs.}
%\label{sec:solvingODE}
We present the explicit solution of the ODEs 
in the case of two clusters ($m=2$) with opposite mean vectors $\pm {\pmb v}$, as %presented 
in \cite{mannelli2022unfair}.
Henceforth,  we refer to $\pmb v$ as the shift vector and to the two clusters as the `positive' and `negative' sub-populations, with mixing probabilities $\rp$ and $\rn$, variances $\Delta_\pm$ and teacher vectors $\overline{\w}_\pm$, respectively. 
The order parameters introduced in Eq.~\ref{eq:oparam} are  specifically denoted as $M = \w^\top\v/d$, $R_+ = \w^\top\overline{\w}_+/d$, and $R_- = \w^\top\overline{\w}_-/d$ in this setting. 

\begin{theorem}\label{thm:sol_ODEs}
In the above setting, solutions to the order parameter evolution  take the form 
\begin{align}
\label{eq:Mt_exact}
    M(t) &= M_0e^{-\eta(v+\Delta^{mix})t} + M^{\infty}(1-e^{-\eta(v+\Delta^{mix})t}), \\
    \label{eq:Rt_exact}
    R_\pm (t) &= R_\pm^0 e^{-\eta\Delta^{mix}t} + R_\pm^{\infty}(1-e^{-\eta\Delta^{mix}t}) + k^\pm_1 ( e^{-\eta\Delta^{mix}t} - e^{-\eta(v+\Delta^{mix})t}), \\
    \label{eq:Qt_exact}
    Q(t) &= Q_0e^{-\eta(2\Delta^{mix} - \eta\Delta^{2mix})t} + Q^{\infty}(1-e^{-\eta(2\Delta^{mix} - \eta\Delta^{2mix})t}) \nonumber \\ 
         &+ k_2 (e^{-t(2\Delta^{mix} - \eta\Delta^{2mix})\eta} - e^{-t\Delta^{mix}\eta}) 
         + k_3 (e^{-t(2\Delta^{mix} - \eta\Delta^{2mix})\eta} - e^{-t(v+\Delta^{mix})\eta}) \nonumber \\
         &+ k_4 (e^{-t(2\Delta^{mix} - \eta\Delta^{2mix})\eta} - e^{-t(2v+2\Delta^{mix})\eta}),
\end{align}
with  $\Delta^{mix} = \rho\Delta_+ + (1-\rho)\Delta_-$, $\Delta^{2mix} = \rho\varp^2 + (1-\rho)\varn^2$ and $v = ||\v||^2/d$. 
\end{theorem} 
The remaining constants are less significant and are reported in Appendix~\ref{sec:appendix_ode_soln} and discussed further in Appendix~\ref{sec:appendix_more_insights}.
%
This solution allows us to describe important observables such as the generalisation error %(via Lemma \ref{thm:gen_error}) 
at any timestep. 
Fig.~\ref{fig:TM_illustration}a plots the theoretical closed-form solutions along with values obtained through %actual 
simulation when we set $d=1000$.  Note the remarkable agreement between the analytical ODE solution and simulations of the online SGD dynamics in this high dimensional data limit.
%\footnote{We provide code to simulate the dynamics and and plot the analytic solution at the following URL}. 
%in the supplementary material.


\begin{wrapfigure}{r}{0.41\textwidth}
    \vspace{-1.2cm}
    \centering
    \includegraphics[width=0.4\columnwidth]{NeurIPS2024/figures/spurious_phases_no_legend.pdf}
    %\vspace{-0.5cm}
    \caption{
    \textbf{Spurious correlations transient alignment.}
    Time-evolution of loss (purple), student-teacher (red) and student-shift (green) cosine similarities.  
    The initial phase (green background) of learning aligns classifier and shift vector before aligning with the teacher (red background). %Sec.~\ref{sec:spurious}. 
    Parameters: $v= 16, \rho=0.5, \varn=\varp=0.1, T_\pm=1, \eta=0.5$. %For these parameters, spurious features allow the correct classification of 90\% of the samples.
    \label{fig:spurious_correlations}
    }
    \vspace{-1.7cm}
\end{wrapfigure}


\section{Insights}\label{sec:insights}
 %In this section, we delve deeper into the solution derived in Theorem \ref{thm:sol_ODEs}. 
 By examining the exponents in Eqs.~\ref{eq:Mt_exact}-\ref{eq:Qt_exact},  we can identify the relevant training timescales. Notably,  $M$ follows a straightforward behaviour dominated by a single timescale,  whereas $R_\pm$ and $Q$ exhibit multiple timescales, leading to significant implications for the emergence and evolution of bias during training. 
 
 
 %In the following sections,  we analyse increasingly complex scenarios to understand how bias develops and evolves. 
 Parameters specifying these different bias scenarios are the shift norm $v = ||\v||^2/d$  and relative representation $\rho$, the subpopulation variances $\Delta_\pm$, and the teacher overlap $T_{\pm} = \wtp^\top \wtn / d$. For simplicity we fix the teacher norm $\|\w_\pm\|_2 = \sqrt{d}$, so that $T_\pm$ is the cosine similarity between the two teachers. 

\subsection{Spurious correlations}\label{sec:spurious}
The emergence of spurious correlations during training illustrates a type of bias where a classifier favours a spurious feature over a core one. To isolate the impact of spurious correlation in our model while avoiding confounding effects, we consider perfectly overlapping teachers ($\wtp = \wtn$) and sub-populations with equal variance and representation ($\rp=0.5, \varp=\varn$). With non-perfectly overlapping clusters $v\neq0$, we introduce a spurious correlation by adding a small cosine similarity between the shift vector and the teacher, creating 
a label imbalance within each sub-population (Fig.~\ref{fig:TM_illustration}b).  
 %---an imbalance between the proportion of positive and negative labels---
%The setting is illustrated in Fig.~\ref{fig:TM_illustration}b. 

From Eqs.~\ref{eq:Mt_exact}-\ref{eq:Qt_exact}, two relevant timescales for the problem are observed:
%\begin{align}
\begin {equation}
    \label{eq:t_M&t_R}
    \tau_M = \frac1{\eta(v+\Delta^{mix})}, \qquad
    %\label{eq:t_R}
    \tau_R = 1/\eta\Delta^{mix}.
%\end{align}
\end{equation}
The shortest timescale, $\tau_M$, %associated with $M$, 
indicates that the student first aligns with the spurious feature. By aligning with the shift vector, 
the student can predict most  examples correctly, but not all.  The effect of spurious correlations is transient; at $t\sim\tau_R$,  the student starts disaligning from the spurious feature and aligns with the teacher vector,  eventually achieving nearly perfect alignment (Fig.~\ref{fig:spurious_correlations}). 
%This is illustrated in Fig.~\ref{fig:spurious_correlations}, where the student initially picks up on the spurious correlation  (green) and achieves almost perfect alignment with the shift vector during intermediate times before aligning nearly perfectly with the teacher (red).

\subsection{Fairness}\label{sec:fairness}

In this section,  we identify the properties of sub-populations that determine the bias during learning and show how bias evolves in three phases.
% 
To quantify bias, we use the \textit{overall accuracy equality} metric~\cite{berk2021fairness}, which measures the discrepancy in accuracy across groups. Intuitively, we aim for equal loss on both groups, considering  any deviation from this condition as bias.

\begin{figure*}[t]
    \vskip 0.2in
    \centering
    \begin{subfigure}[b]{0.63\columnwidth}
        \includegraphics[width=\columnwidth]{NeurIPS2024/figures/single_crossing.pdf}
        \vspace{-0.7cm}
        \caption{Bias crossing}
    \end{subfigure}
    \begin{subfigure}[b]{0.36\columnwidth}
        \includegraphics[width=\columnwidth]{NeurIPS2024/figures/fairness_crossing_heatmap.pdf}
        \vspace{-0.6cm}
        \caption{Crossing phase diagram}
    \end{subfigure}
    \caption{
        \textbf{The crossing phenomenon.} \textit{Panel (a) (left side)} shows the loss curves of sub-population $-$ (in red) and sub-population $+$ in blue along with the overall loss (in purple). We observe a crossing cause by a higher variance but lower representation in sub-population $-$. 
        The background colours represent the different phases of bias that are characterised by the evolution of the order parameters shown in \textit{Panel (a) (right side)}.
        \textit{Panel (b)} shows the presence of the crossing phenomenon in a large portion of the parameter space using a phase diagram. Blue indicates an asymptotic preference for sub-population $+$ and red the opposite. Dark colours indicates regions where bias is consistent across training, while regions in light colours undergo a crossing phenomenon. White indicates that learning rate was too high and training diverged. Parameters: $v=0, \varp=1, T_\pm=0.9, \eta=0.1$.        
    }
    \label{fig:fairness_crossing}
\vskip -0.2in
\end{figure*}

\textbf{Zero shift.}
We first consider a simplified case where we assume that both clusters are centered at the origin $v = 0$ as shown in Fig.~\ref{fig:TM_illustration}c. We will later reintroduce the shift and analyse the transient dynamics it introduces as per the discussion in section \ref{sec:spurious}. This setting is particularly suited to analysing the effects of `group level' features, such as group variance and relative representation, on the preference of the classifier. 

In this simplified setting, $M(t)$ is always zero and the constants $k_1^\pm, k_3, k_4$ presented in equations~\ref{eq:Rt_exact} and~\ref{eq:Qt_exact} are zero. 
Thus, the dynamics only involve two relevant timescales given by $\tau_R$ in Eq.~\ref{eq:t_M&t_R} and
\begin{align}
    & \tau_Q = 1/(\eta(2\varmix-\eta\varmixsq)). \label{eq:t_Q}
\end{align}

Fig.~\ref{fig:fairness_crossing}a illustrates the changing preference of the classifier. Specifically, we observe that the variance of the sub-population is particularly relevant initially and the sub-population with higher variance (red) is \textit{learnt} faster, i.e. its generalisation error drops faster. However, asymptotically we observe that the relative representation becomes more important wherein the student aligns itself with the teacher that has a higher product of representation and standard deviation (blue), i.e. 
\begin{equation}
    \label{eq:asymptotic_metric}
     \rp\sqrt{\varp} \gtrless \rn\sqrt{\varn} \iff R_+^\infty \gtrless R_-^\infty.
\end{equation}
Thus, the network can advantage the cluster with higher variance initially but asymptotically advantage the other cluster if its representation is high enough. This leads to the `crossing' of the losses on the two sub-populations shown in  Fig.~\ref{fig:fairness_crossing} (more in Appendix ~\ref{sec:appendix_detailed_fairness}).

\uline{\emph{Initial dynamics.}}
The ratio between initial rate of change in generalisation errors is bounded by (derived in Appendix \ref{sec:appendix_initial_rates}):
\begin{equation}
    \label{eq:initial learning rate}
    T_\pm\sqrt{\frac{\varp}{\varn}} \leq \frac{d\epsilon_{g+}/dt\big|_{t=0}}{d\epsilon_{g-}/dt\big|_{t=0}} \leq \frac{1}{T_\pm}\sqrt{\frac{\varp}{\varn}}.
\end{equation}
When the teachers are only slightly misaligned---$T_\pm\lessapprox1$---the bound is tight and we can see that it is the ratio of the square roots of the variances that determines which cluster is learnt faster initially.
Fig.~\ref{fig:fairness_crossing}b shows in a phase diagram the existence of `bias crossing' across a wide range of variances and representations. The transition between the phases that represent a initial preference for the positive sub-population (light red and dark blue) and the phases that represent an initial preference for negative sub-population (dark red and light blue) is approximately given by the line $\varn = \varp = 1$, independent of the representation as predicted by Eq.~\ref{eq:initial learning rate}. The portion of the dark blue phase just above the white divergent phase marks a `quasi-divergent' region wherein the generalisation error on the negative sub-population rises even at $t=0$ because the learning rate is too large for such high variances and marks a region of impractical behaviour observed with poorly optimised learning rates.

\uline{\emph{Asymptotic preference.}}
In the limit of small learning rates $\eta \rightarrow 0$, the student will asymptotically exhibit lower loss on whichever sub-population's teacher it has better alignment with. 
Thus, Eq.~\ref{eq:asymptotic_metric} provides a simple characterisation of asymptotic preference from representations and standard deviations in the small learning rate limit.
However, the situation is more complex in the case of finite learning rate, which may disrupt learning in one or both clusters (more in Appendix~\ref{sec:appendix_more_insights_asymptotic}). 
%Without indulging further into the discussion of asymptotic performance, which is not the main goal of the paper, 
%we refer to Appendix~\ref{sec:appendix_more_insights_asymptotic} for more in depth and analysis and additional phase diagrams. 

% 
\begin{wrapfigure}{r}{0.6\textwidth}
    \vspace{-0.5cm}
    \centering
    \includegraphics[width=0.59\columnwidth]{NeurIPS2024/figures/triple_crossing.pdf}
    \vspace{-0.2cm}
    \caption{
        \textbf{Double crossing phenomenon.}
        \textit{(Left panel)} shows the loss for the two sub-populations (blue and red lines) and the global one (in purple). \textit{(Right panel)} shows the value of the order parameters across time. The behaviour of the order parameters across time provides a precise characterisation and understanding of the different phases. Parameters: $v = 100, \rho = 0.75, \varp=0.1, \varn = 0.5, \eta = 0.03, T_\pm = 0.9, \alphap = 0.343, \alphan = 0.12$.
    }
    \vspace{-0.3cm}
    \label{fig:double_crossing}
\end{wrapfigure}
% 
\textbf{General case.}
We now consider the general case shown in Fig.~\ref{fig:TM_illustration}d, where the shift is non zero and all three timescales identified so far play a role. 

As observed in Sec.~\ref{sec:spurious}, when the shift norm $v$ is large, the effect of spurious correlations becomes significant and the timescale associated with the spurious correlations is the fastest. In general, when $v\neq0$ we observe an additional phase due to the effect of spurious correlation. In this new first phase, the student advantages the cluster with higher representation and lower variance since the salient information received from this cluster is more coherent and easier to access. 

More precisely, in high dimensions the shift and the teachers are likely to exhibit a small cosine similarity leading to a class imbalance in the clusters and creating spurious correlation. The amount of label imbalance within a cluster is characterised by the value of $\alpha$, as detailed in Appendix~\ref{sec:appendix_notation}. 
For smaller variances, $\alpha$ takes more extreme values leading to stronger spurious correlation of that cluster with the shift. 
If a cluster has more positive examples, we would observe a reduction in loss for that cluster if the student aligns with the mean of that cluster (and opposite to the mean if the cluster has mostly negative examples). When both clusters have different majority classes, the direction of spurious correlation for the two are same. However, when the majority classes are the same, we have competing directions for spurious correlation. The expression for $M_\infty$ in Appendix~\ref{sec:appendix_ode_soln} Eq.~\ref{eq:appendix Minf} shows that in this case the relative representation comes into play and the mean of the cluster with greater representation and class imbalance will be chosen by the teacher to align with. Fig.~\ref{fig:double_crossing} shows such a scenario with three phase bias evolution. First, the green phase is driven by spurious correlation where the positive cluster is advantaged since it has greater representation and class imbalance. Next, the red phase is driven by greater variance where the negative cluster is learnt faster as discussed through Eq.~\ref{eq:initial learning rate}. Finally, we observe the orange phase wherein the student starts aligning with the positive cluster as per the asymptotic rule in Eq.~\ref{eq:asymptotic_metric}.

%In summary, the student first advantages the sub-population with higher representation and lower variance. Next, it advantages the sub-population with higher variance. Asymptotically, it advantages the sub-population with higher representation and variance. 
Our analysis thus shows that bias is a dynamical quantity that can vary non-monotonically during training and cannot be characterised by simply the initial and asymptotic values.

\section{Ablations using numerical simulations}\label{sec:numerical_simulations}

\begin{wrapfigure}{r}{0.61\textwidth}
    \vspace{-0.7cm}
    \centering
    \begin{subfigure}[b]{0.30\columnwidth}
        \includegraphics[width=\columnwidth]{NeurIPS2024/figures/MNIST_crossing.pdf}
        \vspace{-0.8cm}
        \caption{Crossing phenomenon}
    \end{subfigure}
    \begin{subfigure}[b]{0.30\columnwidth}
        \includegraphics[width=\columnwidth]{NeurIPS2024/figures/MNIST_double.pdf}
        \vspace{-0.8cm}
        \caption{Double crossing phenomenon}
    \end{subfigure}
    \caption{
        \textbf{Numerical simulations on MNIST.}
        The figure shows the average (solid lines) and standard deviation (shaded area) of 100 simulations run in this framework. In particular the upper plots show the test loss and lower plots the test accuracy for subpopulation $+$ (blue) and $-$ (red).
        \textit{Panel (a)} an example of crossing phenomenon obtained by imposing $\sqrt\Delta_+=1$, $\sqrt\Delta_-=0.2$, and $\rho=0.1$. 
        \textit{Panel (b)} shows the double crossing, obtained by introducing an additional timescale to the previous case by tuning label imbalance.
    }
    \label{fig:numerical_experiments_MNIST}
    \vspace{-0.2cm}
\end{wrapfigure}

\textbf{Rotated MNIST.}
% 
We train a 2-layer neural network with 200 hidden units, ReLU activation, and sigmoidal readout activation %, using online SGD on MSE loss 
on a variation of MNIST %classification task. 
%Data are centered and the variance is set to 1 following standard pre-processing practices. 
%We consider a variation of the MNIST dataset 
that mimics our model.  
%allowing us to verify our theory when network and the data structure are mismatched. 
Digits 0 to 4 and 5 to 9 are grouped to form the two subpopulations. With probability $p_+$ and $p_-$, digits of both subpopulations are rotated with a subpopulation-specific angle---i.e. Fig.~\ref{fig:numerical_experiments_MNIST}a uses angles of rotation $\theta_-=45^o$ and $\theta_-=-90^o$. The goal of the classifier is to detect rotations.

The experimental framework gives a correspondence between parameters of the generative model and properties of a real dataset. We can control relative representation by subsampling, teacher similarity by playing with angle difference, label imbalance by changing the probability of rotation, and saliency by increasing and decreasing the norm of the subpopulation using multiplicative factors $\Delta_\pm$. The only parameter that we cannot control is the shift $\v$ which is a property of the data. 

Therefore, in order to reproduce the zero-shift case of Sec.~\ref{sec:fairness}, we remove the label imbalance by setting the probability of rotation $p_+=p_-=0.5$.
By properly calibrating the saliency $\Delta$ and the relative representation $\rho$, it is possible to bias the classifier towards one subpopulation at the beginning of training and the other in the end. This is shown in Fig.~\ref{fig:numerical_experiments_MNIST}a where $\rho=0.1$ and $\Delta_+>\Delta_-$. The saliency difference favours subpopulation $+$ initially while setting $\rho$ small enough advantages subpopulation $-$ later in training. This is precisely what we observe in the plot. 

Finally, we consider the general fairness case. By creating label imbalance, i.e. setting $p_+=0.3$ and $p_-=0.7$, we observe an additional phase of bias evolution, wherein the classifier prefers dense regions with consistent labels. This advantages subpopulation $-$ and indeed it is what we see in Fig.~\ref{fig:numerical_experiments_MNIST}b. The result of the simulations matches the theory displaying a double crossing phenomenon.

\textbf{Additional numerical expirements.} In Appendix~\ref{sec:appendix_more_numerical_simu}, we provide additional experiments within our model and the CIFAR10 and CelebA, exploring different architectures and losses. We observe that bias presents different timescales and shows crossing behaviors. 


\section{Conclusion}\label{sec:conclusion}

This paper examined the dynamics of bias in a high dimensional synthetic framework, showing that it can be explicitly characterised to  reveal transient behaviour. Our findings reveal that classifiers exhibit biases toward different data features during training, possibly alternating sub-population preference. Although our analysis is based on certain assumptions, 
numerical experiments that violate these assumptions still display the behaviour predicated by our theory. 
%Future research will explore the limitations of our theory with more complex classifiers and richer data structure.



%While this paper centered on bias propagation in a controlled synthetic setting, the study of bias in ML systems is a significant issue with profound societal implications. 
We believe 
this line of research will have  practical impacts in the medium term, aiding the design of mitigation strategies that account for transient dynamics. Future research will further explore this connection,  proposing theory-based dynamical protocols for bias mitigation.

